A Survey on Deep Learning Hardware Accelerators for Heterogeneous HPC Platforms

Recent trends in deep learning (DL) have made hardware accelerators essential for various high-performance computing (HPC) applications, including image classification, computer vision, and speech recognition. This survey summarizes and classifies the most recent developments in DL accelerators, focusing on their role in meeting the performance demands of HPC applications. We explore cutting-edge approaches to DL acceleration, covering not only GPU- and TPU-based platforms but also specialized hardware such as FPGA- and ASIC-based accelerators, Neural Processing Units, open hardware RISC-V-based accelerators, and co-processors. This survey also describes accelerators leveraging emerging memory technologies and computing paradigms, including 3D-stacked Processor-In-Memory, non-volatile memories like Resistive RAM and Phase Change Memories used for in-memory computing, as well as Neuromorphic Processing Units, and Multi-Chip Module-based accelerators. Furthermore, we provide insights into emerging quantum-based accelerators and photonics. Finally, this survey categorizes the most influential architectures and technologies from recent years, offering readers a comprehensive perspective on the rapidly evolving field of deep learning acceleration.

==> images/riscv_table_old.tex <==
\begin{table}[bt]
\caption{Summary of RISC-V Deep Learning acceleration architectures}
\label{tab:riscv}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllrrrrrrrll@{}}
\toprule
\textbf{Category} & \textbf{Accelerator}                                                                             & \textbf{Tech [nm]} & \multicolumn{1}{l}{\textbf{Area [mm2]}} & \multicolumn{1}{l}{\textbf{Freq [MHz]}} & \multicolumn{1}{l}{\textbf{Voltage [V]}} & \multicolumn{1}{l}{\textbf{Power [mW]}} & \multicolumn{1}{l}{\textbf{Perf [GOPS]}} & \multicolumn{1}{l}{\textbf{Eff [GOPS/W]}} & \multicolumn{1}{l}{\textbf{\# MAC units}} & \textbf{Data Type} & \textbf{Maturity} \\ \midrule
\multirow{8}{*}{\textbf{ISA}} & Dustin \cite{ottaviDustin16CoresParallel2023}                                                    & 65nm               & 10                                      & 205                                     & 1.2                                      & 156                                     & 33.6                                     & 215                                                     & 128                                      & INT2 x INT4        & Silicon           \\
& Kraken (RISC-V cores) \cite{dimauroKrakenDirectEvent2022}                                                      & 22nm               & 9                                       & 330                                     & 0.8                                      & 300                                     & 75                                       & 750                                                     & 128                                      & INT2               & Silicon           \\
& Manticore \cite{zarubaManticore4096CoreRISCV2021}                                                & 22nm               & 888                                     & 500                                     & 0.6                                      & 200                                     & 25                                       & 188                                                     & 24                                       & FP64               & Silicon           \\
& Celerity \cite{davidsonCelerityOpenSource511Core2018}                                            & 16nm               & 25                                      & 1050                                    & -                                        & 1900                                    & -                                        & -                                                       & 496                                      & INT32              & Silicon           \\
& Tenstorrent \cite{vasiljevicComputeSubstrateSoftware2021}                                        & 12nm               & 477                                     & -                                       & -                                        & -                                       & 92000                                    & -                                                       & -                                        & FP16               & Silicon           \\
& exSDOTP \cite{bertacciniMiniFloatNNExSdotpISA2022}                                               & 12nm               & 0.52                                    & 1260                                    & 0.8                                      & \textit{278}                            & 160                                      & 575                                                     & 16                                       & FP8                & Pre-silicon       \\
& Esperanto \cite{ditzelAcceleratingMLRecommendation2022}                                          & 7nm                & 570                                     & 1000                                    & -                                        & 20000                                   & 139000                                   & 6.95                                                    & 69632                                    & INT8               & Silicon           \\
& CNC \cite{chenEightCoreRISCVProcessor2022}                                                       & 4nm                & 1.92                                    & 1150                                    & 0.85                                     & 510                                     & 75.8                                     & 149                                                     & 512                                      & INT8               & Silicon           \\ \midrule
%
\multirow{6}{*}{\textbf{Vector}} & Lee et al. \cite{lee64TOPSEnergyEfficientTensor2022}                                             & 14nm               & 181                                     & 2000                                    & 0.8                                      & 60000                                   & 64000                                    & 1450                                                    & 16384                                    & INT8               & Silicon           \\
& AVA \cite{lazoAdaptableRegisterFile2022}                                                         & 22nm               & 3.9                                     & -                                       & -                                        & -                                       & -                                        & -                                                       & -                                        & FP64               & Pre-silicon       \\
& Spatz \cite{cavalcanteSpatzCompactVector2022}                                                    & 22nm               & 20                                      & 594                                     & 0.8                                      & 1070                                    & 285                                      & 266                                                     & 256                                      & INT32              & Pre-silicon       \\
& Vitruvius+ \cite{minerviniVitruviusAreaEfficientRISCV2023}                                       & 22nm               & 1.3                                     & 1400                                    & 0.8                                      & 459                                     & 21.7                            & 47.3                                                    & 8                                        & FP64               & Pre-silicon       \\
& Ara \cite{cavalcanteAra1GHzScalable2020}                                                         & 22nm               & 10735 kGE                               & 1040                                    & 0.8                                      & 794                                     & 32.4                                     & 40.8                                                    & 16                                       & FP64               & Pre-silicon       \\
& Perotti et al. \cite{perottiNewAraVector2022}                                                    & 22nm               & 0.81                                    & 1340                                    & 0.8                                      & 280                                     & 10.4                                     & 37.1                                                    & 4                                        & FP64               & Pre-silicon       \\ \midrule
% 
\multirow{7}{*}{\textbf{L1 NPU}} & Darkside \cite{garofaloDARKSIDEHeterogeneousRISCV2022}                                           & 65nm               & 3.85                                    & 200                                     & 1.2                                      & 89.1                                    & 12.6                                     & 152                                                     & 32                                       & FP16               & Silicon           \\
& Marsellus (NPU) \cite{conti22124TOPS2023}                                                        & 22nm               & 18.7                        & 420                                     & 0.8                                      & 123                                     & 637                                      & 7600                                                    & 10368 1--bit                             & INT2               & Silicon           \\
& Garofalo et al. \cite{garofaloHeterogeneousInMemoryComputing2022}                                & 22nm               & 30                                      & 500                                     & 0.8                                      & 150                                     & 958                                      & 6390                                                    & 36 (DW)                                  & INT8               & Pre-silicon       \\
& Vega \cite{rossiVegaTenCoreSoC2022}                                                              & 22nm               & 12                                      & 450                                     & 0.8                                      & 49.4                                    & 32.2                                     & 651                                                     & 27                                       & INT8               & Silicon           \\
& RedMulE \cite{tortorellaRedMuleMixedPrecisionMatrixMatrix2023,tortorellaRedMulECompactFP162022a} & 22nm               & 0.73                                    & 613                                     & 0.8                                      & 193                                     & 117                                      & 608                                                     & 96                                       & FP16               & Pre-silicon       \\
& Archimedes \cite{prasadSpecializationMeetsFlexibility}                                           & 22nm               & 3.38                                    & 270                                     & 0.65                                     & 112                                     & 1198                                     & 10.6                                                    & 5184                                     & INT2 x INT8        & Pre-silicon       \\
& Bruschi et al. \cite{bruschiEndtoEndDNNInference2022}                                            & 5nm                & 480                                     & -                                       & -                                        & 3070                                    & 20000                                    & 6500                                                    & 3.35$\times$10${}^{7}$                   & Analog             & Simulation        \\ \midrule
% 
\multirow{9}{*}{\textbf{L2 NPU}} & SNCPU \cite{juSystolicNeuralCPU2023}                                                             & 65nm               & 4.47                                    & 400                                     & 1                                        & 116                                     & 75.9                                     & 655                                                     & 100                                      & INT8               & Silicon           \\
& SamurAI \cite{miro-panadesSamurAIVersatileIoT2022}                                               & 28nm               & 4.52                                    & 350                                     & 0.9                                      & 94.7                                    & 36                                       & 380                                                     & 64                                       & INT8               & Silicon           \\
& Gemmini \cite{gencGemminiEnablingSystematic2021}                                                 & 22nm               & 1.03                                    & 1000                                    & -                                        & -                                       & -                                        & -                                                       & 256                                      & INT8               & Pre-silicon       \\
& DIANA (digital) \cite{houshmandDIANAEndtoEndHybrid2023}                                          & 22nm               & 10.24                                   & 280                                     & 0.8                                      & 132                                     & 230                                      & 1740                                                    & 256                                      & INT8               & Silicon           \\
& DIANA (analog) \cite{houshmandDIANAEndtoEndHybrid2023}                                           & 22nm               & 10.24                                   & 350                                     & 0.8                                      & 132                                     & 18100                                    & 176000                                                  & 256                                      & INT8               & Silicon           \\
& TinyVers \cite{jainTinyVersTinyVersatile2023}                                                    & 22nm               & 6.25                                    & 150                                     & 0.8                                      & 20                                      & 17.6                                     & 863                                                     & 64                                       & INT8               & Silicon           \\
& Simba \cite{shao_micro19}                                                    & 16nm               & 6                                       & 161                                     & 0.42                                     & -                                       & -                                        & 9100                                                    & 1024                                     & INT8               & Silicon           \\
& Axelera AI \cite{ward-foxtonAxeleraDemosAI}                                                      & 12nm               & 9                                       & 800                                     & -                                        & 2787                                    & 39300                                    & 14100                                                   & -                                        & INT8               & Silicon           \\
& Tambe et al. \cite{tambe2212nm182023}                                                            & 12nm               & 4.59                                    & 717                                     & 1                                        & 111                                     & 734                                      & 6612                                                    & -                                        & FP4                & Silicon           \\ \midrule
% 
\multirow{2}{*}{\textbf{L3 NPU}} & Gonzalez et al. \cite{gonzalez16mm106GOPS2021}                                                   & 22nm               & 16                                      & 961                                     & -                                        & -                                       & -                                        & 106.1                                                   & 256                                      & INT8               & Silicon           \\
& ESP \cite{jia12nmAgileDesignedSoC2022}                                                           & 12nm               & 21.6                                    & 1520                                    & 1                                        & 1830                                    & -                                        & -                                                       & 3x NVDLA                                 & INT8               & Silicon           \\
\bottomrule
\end{tabular}
}
\end{table}

==> sections/sec_cross-sectional.tex <==
\section{Cross-Sectional Design Techniques}

\input{sections/ssec_RISC-V}
\input{sections/ssec_Multi-chip}
